Teaching Embodied Reinforcement Learning Agents: Informativeness and Diversity of Language Use

In real-world scenarios, it is desirable for embodied agents to have the ability to leverage human language to gain explicit or implicit knowledge for learning tasks. Despite recent progress, most previous approaches adopt simple low-level instructions as language inputs, which may not reflect natural human communication. It's not clear how to incorporate rich language use to facilitate task learning. To address this question, this paper studies different types of language inputs in facilitating reinforcement learning (RL) embodied agents. More specifically, we examine how different levels of language informativeness (i.e., feedback on past behaviors and future guidance) and diversity (i.e., variation of language expressions) impact agent learning and inference. Our empirical results based on four RL benchmarks demonstrate that agents trained with diverse and informative language feedback can achieve enhanced generalization and fast adaptation to new tasks. These findings highlight the pivotal role of language use in teaching embodied agents new tasks in an open world. Project website: https://github.com/sled-group/Teachable_RL

==> figures/data_collection_algo.tex <==
\begin{algorithm*}[h]
\caption{Offline Data Collection}
\label{alg:data_collection}
\begin{algorithmic}[1]
\State Initialize $\mathcal{D} \leftarrow \emptyset$

\For{each episode with $seed_i$}
    \State Initialize $\mathcal{D}_i \leftarrow \emptyset$
    \State Initialize environment simulator $env$ with $seed_i$.
    \State Append task description $Td$ to $\mathcal{D}_i$
    \State Initialize the agent with policy $\pi$.
    \State Initialize the expert agent with optimal policy $\pi^{*}$.
    
    \For{each time step}
        \State Get action from agent $a_t \leftarrow \pi(r_{t-1}, s_{t-1}, a_{t-1})$
        \State Get action from expert agent $a^{*}_t \leftarrow \pi^{*}(r_{t-1}, s_{t-1}, a_{t-1})$
        \State Step environment $r_t, s_t, l_t^{hind}, l_t^{fore} \leftarrow \text{env}(a_t| a^{*}_t )$.
        \If{Use GPT Template Pool}
            \State $l_t^{hind}=\text{RandomChoice}(\text{TemplatePool}[l_t^{hind}])$
            \State $l_t^{fore}=\text{RandomChoice}(\text{TemplatePool}[l_t^{fore}])$
        \EndIf
        \State Get language feedback $l_t \gets \left\{
        \begin{array}{ll}
        \text{concat}(l_t^{\text{hind}}, l_t^{\text{fore}}) & \text{if Hindsight + Foresight} \\
        l_t^{\text{hind}} & \text{if only Hindsight} \\
        l_t^{\text{fore}} & \text{if only Foresight} \\
        \text{<empty string>} & \text{if No Lang}
        \end{array}
        \right.$
        \State Append $(r_t, s_t, a_t, l_t)$ to $\mathcal{D}_i$
    \EndFor
    \State Aggregate Datasets $\mathcal{D} \leftarrow \mathcal{D}\cup\mathcal{D}_i$
\EndFor

\end{algorithmic}
\end{algorithm*}

==> figures/feedback_evaluation_generation.tex <==
\usetikzlibrary{arrows.meta, positioning}

\begin{tikzpicture}[>=Stealth, node distance=4cm, auto, ultra thick]

% First graph (left)
\begin{scope}

    % Nodes
    \node[draw, circle, minimum width=3cm, minimum height=3cm, align=center, font=\Large, scale=1.5] (agent1) {Agent\\with\\policy $\pi$};
    \node[draw, circle, minimum width=3cm, minimum height=3cm, align=center, above=2cm of agent1, font=\Large, scale=1.5] (env1) {Environment\\Simulator};
    \node[font=\Large, align=center, below=1cm of agent1, scale=2.5, baseline] (legend1) {Data Collection};
    
    % Arrows
    \draw[->, bend left, font=\Large] (agent1) to node[left, scale=2] {$a_t$} (env1);
    \draw[->, bend left, font=\Large] (env1) to node[right, font=\huge, align=center, text width=3cm, scale=1.5] {$r_t, s_t$, $l_t$ } (agent1);

\end{scope}

% Second graph (right)
\begin{scope}[shift={(10cm, 0)}] % Shift the second graph to the right

    % Nodes
    \node[draw, circle, minimum width=3cm, minimum height=3cm, align=center, font=\Large, scale=1.5] (agent2) {Agent\\with\\policy $\pi$};
    \node[draw, circle, minimum width=3cm, minimum height=3cm, align=center, above right=3cm and 1.5cm of agent2, font=\Large, scale=1.5] (env2) {Environment\\Simulator};
    \node[draw, circle, minimum width=3cm, minimum height=3cm, align=center, right=4cm of agent2, font=\Large, scale=1.5] (gpt2) {Online \\ GPT};
    \node[font=\Large, align=center, below=7.27cm of env2, scale=2.5] (legend2) {Evaluation};
    
    % Arrows
    \draw[->, bend left, font=\Large] (agent2) to node[sloped, above, scale=2] {$a_t$} (env2);
    \draw[->, bend left, font=\Large] (env2) to node[sloped, below, scale=2] {$r_t, s_t$} (agent2);
    \draw[->, font=\Large] (env2) -- node[right, scale=2] {$l_t^{hind}, l_t^{fore}$} (gpt2);
    \draw[->, font=\Large] (gpt2) -- node[sloped, below, scale=2] {$l_t$} (agent2);
\end{scope}

\end{tikzpicture}


==> figures/feedback_generation_tex.tex <==
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}

\begin{tikzpicture}[>=stealth, node distance=5.5cm, ultra thick]



\fill[green!8, rounded corners=10pt] (-2,3) rectangle (13,7);
\fill[red!8, rounded corners=10pt] (-2,-2) rectangle (13,2);
\fill[white, draw=black, dashed, rounded corners=10pt] (1,-2.3) rectangle (15,-4);
\fill[white, draw=black, dashed, rounded corners=10pt] (1,-4.7) rectangle (15,-7);
% Adding gpt figure to top left of specified rectangle
\node[rectangle, minimum width=2cm, minimum height=2cm, align=center, anchor=north west] at (0,-3.7) {\includegraphics[width=1cm,height=1cm]{figures/gpt.pdf}};
% Nodes
\node[draw, rectangle, minimum width=3cm, minimum height=3cm, align=center] (frame1) {\includegraphics[width=3cm,height=3cm]{figures/figs_feedback_gen/frame1.pdf}};
\node[draw, rectangle, minimum width=3cm, minimum height=3cm, align=center, right of=frame1] (frame2) {\includegraphics[width=3cm,height=3cm]{figures/figs_feedback_gen/frame2.pdf}};
\node[draw, rectangle, minimum width=3cm, minimum height=3cm, align=center, right of=frame2] (frame3) {\includegraphics[width=3cm,height=3cm]{figures/figs_feedback_gen/frame3.pdf}};
\node[draw, rectangle, dashed, minimum width=3cm, minimum height=3cm, align=center, above of=frame1, node distance=5cm] (frame4) {\includegraphics[width=3cm,height=3cm]{figures/figs_feedback_gen/frame4.pdf}};
\node[draw, rectangle, dashed, minimum width=3cm, minimum height=3cm, align=center, above of=frame2, node distance=5cm] (frame5) {\includegraphics[width=3cm,height=3cm]{figures/figs_feedback_gen/frame5.pdf}};
\node[draw, rectangle, dashed, minimum width=3cm, minimum height=3cm, align=center, above of=frame3, node distance=5cm] (frame6) {\includegraphics[width=3cm,height=3cm]{figures/figs_feedback_gen/frame6.pdf}};

% Arrows
\draw[->] (frame1) -- node[below, scale=2] {$a_t$} (frame2);
\draw[->] (frame1) -- node[above, scale=1.5] {"up"} (frame2);
\draw[->] (frame2) -- node[below, scale=2] {$a_{t+1}$} (frame3);
\draw[->] (frame2) -- node[above, scale=1.5] {"down"} (frame3);
\draw[->, dashed] (frame1) -- node[left, scale=2] {$a_t^*$} (frame4);
\draw[->, dashed] (frame1) -- node[right, scale=1.5] {"pedal"} (frame4);
\draw[->, darkgreen, dashed] (frame2) -- node[left, scale=2] {$a_{t+1}^{*}$} (frame5);
\draw[->, darkgreen, dashed] (frame2) -- node[right, scale=1.5] {"down"} (frame5);
\draw[->, darkgreen, dashed] (frame3) -- node[left, scale=2] {$a_{t+2}^{*}$} (frame6);
\draw[->, darkgreen, dashed] (frame3) -- node[right, scale=1.5] {"pedal"} (frame6);
\draw[<->, red, dashed] (frame4) -- (frame2);
\draw[<->, red, dashed] (frame5) -- (frame3);

% Legends
\node[align=center, xshift=-2cm, yshift=-1.5cm] at (frame1.south)(tmp1) {
    \textcolor{black}{Language Feedback Templates} \\
    \textcolor{black}{from environment simulator} 
};
\node[align=left, xshift=-0.5cm, yshift=-1.5cm] at (frame2.south)(t1template) {
    \textcolor{red}{H: You have gone to the wrong direction.} \\
    \textcolor{darkgreen}{F: Turn back.}
};
\node[align=left, yshift=-1.5cm] at (frame3.south)(t2template) {
    \textcolor{red}{H: You are doing well so far.} \\
    \textcolor{darkgreen}{F: Pedal to open the trash bin.}
};

% Legends
\node[align=center, yshift=-2cm] at (tmp1.south)(tmp2) {
    \textcolor{black}{GPT Translated Templates} \\
    \textcolor{black}{from GPT Template Pool} 
};
\node[align=left, xshift=-0.2cm, yshift=-2cm] at (t1template.south) {
    \textcolor{red}{H: You seem to be heading away from} \\
    \textcolor{red}{ the right route.} \\
    \textcolor{darkgreen}{F: Make a 180-degree turn right now.}
};
\node[align=left, xshift=6.7cm, yshift=-2.23cm] at (t1template.south) {
    \textcolor{red}{H: So far, so good, you're doing great!} \\
    \textcolor{red}{} \\
    \textcolor{darkgreen}{F: To access the recycling bin, you'll} \\
    \textcolor{darkgreen}{need to pedal.}
};

% Additional Legends
\node[align=center, left of=frame4, node distance=3.5cm](legend1) {
    \textcolor{black}{Expert Agent $\pi^*$} \\
    \textcolor{black}{Prediction}
};
\node[align=center, left of=frame1, node distance=3.5cm](legend2) {
    \textcolor{black}{Agent $\pi$} \\
    \textcolor{black}{Prediction}
};
\node[align=center, xshift=1cm, yshift=-2cm] at (legend1.south west) {
    \textcolor{black}{\textbf{Task Description:}} \\
    \textcolor{black}{\textbf{Open the recycling bin.}}
};

\draw[->] (tmp1) -- node[left] {GPT Rephrasing} (tmp2);
\end{tikzpicture}


==> rebuttal_EMNLP_24.tex <==
Google Doc link: \url{https://docs.google.com/document/d/1yT8eivuUAh_L2PIX3WM4GimWJ_MnI09PpXfqy2pLPRo/edit#heading=h.ixwf1krxxg8w}

Reviewer 1 AkZT (score 3)
We thank the reviewer for the positive feedback on the merit of this work (e.g., detailed evaluation, sufficient statistics, etc.). We also appreciate valuable comments and suggestions. 
Q1: Not surprising that non-expert agents outperform agents trained from scratch.
A1: Sorry for the confusion. All non-expert agents that are part of the experiments are trained based on different conditions, e.g., pre-training with no language and pre-training with GPT augmented hindsight language, etc. Our goal here is not to compare our non-expert agents with agents that are trained from scratch, but rather we aim to compare different versions of non-expert agents that are trained by using different kinds of language feedback in order to study the role of language use in RL learning. Figure 5 “Train from Scratch” is used as a reference point. As it causes some confusion about our objective, we will remove it from the comparison. Thanks for pointing this out!
Q2: How does hindsight feedback impact decisions in future time steps?
A2: Thank you for this question! Compared to foresight feedback, which provides instructions for the correct action in the next step, hindsight feedback reflects on incorrect actions taken in previous steps. This retrospective analysis can still guide agents toward success by narrowing down the search space for corrective actions.
To demonstrate the effectiveness of hindsight feedback, we conducted a quick comparative study between a no-language agent and a hindsight-only agent in Homegrid. The study was designed as follows:
Both agents were driven to the same state using an expert policy.
A deliberate mistake was introduced for both agents. Three types of mistakes were designed:
Navigation Mistake: The agent moves in the opposite direction compared to the expert action.
Object Pick/Drop Mistake: The agent picks or drops an object when the expert action is to drop or pick, respectively.
Bin manipulation Mistake: The agent chooses the wrong action among pedal/lift/grasp to open a specific trash bin.
We used expert actions as the ground truth (GT) actions and compared the performance of both agents over 500 runs. The results are as follows:
|Mistake Type|	No Lang Agent (%)|	Template Hindsight Agent (%)|
|---|---|---|
|Navigation|	37.6 ± 0.3|	46.2 ± 0.2|
|Object Pick/Drop|	37.4 ± 2.5|	41.8 ± 1.6|
|Bin manipulation|	23.5 ± 1.2|	24.8 ± 0.9|
As we can see, for the navigation and object pick/drop mistakes, hindsight feedback is highly beneficial. This is because identifying a wrong action usually directly implies the correct action for those mistakes (e.g., if "turn left" is wrong, "turn right" is correct; if "pick the object" is wrong, "drop the object" is correct). However, for the bin manipulation mistake, hindsight feedback is less helpful since there are no clear implications for the correct action.
We will clarify this in the revision, thank you! 

>Q3: How many templates? How to chose? and how do they differ?
A3: Thanks for your insightful question! For each environment, we designed several templates conveying different meanings, and then applied GPT to augment the languages. Details are shown below:
| Env |\# hindsight templates | \# foresight templates | \# augmented sentences for each template |
|---|---|---|---|
| HomeGrid | 20 | 9 | 70 |
| AlfWorld | 4 | 4 | 200  |
| Messenger | 4 | 4 | 200 |
| MetaWorld | 2 | 6 | 180  |
The templates were selected by rules to provide agents with diverse types of privileged knowledge.
For instance, in the Messenger, two specific foresight instructions illustrate this approach effectively:
|Foresight Instruction |Privileged knowledge |situation |
|---|---|---|
|“Move {action} to avoid the {enemy} at {loc}” |optimal action, enemy entity, enemy location | agent in danger |
|“Step {action} to approach the {target} at {loc}” |optimal action, target entity, target location | no enemies around | 
More examples can be seen in Appendix A. Thank you for your feedback!
>Q4: How to compare the actions? How this comparison leads to template selection?
A4: We compare the agent’s actions with expert actions and analyze the agent’s task progress and situations. This allows us to determine whether the agent is on the right track and decide which type of privileged knowledge may help the agent. The template is then chosen based on a set of rules. For example, in the Messenger environment, we compare actions, consider the locations of the target and nearest enemy, and generate hindsight reflections. We apologize for any confusion and will elaborate more on this in the revision.
>Q5. We claim the generalizability over unseen tasks. However, the evaluation only contains one unseen task. More clarification is needed.
A5. Thank you for your  suggestion! We will clarify that our current evaluation demonstrates generalization to one unseen task. In the future, we will extend its generalization to more diverse unseen tasks.

Q3: Please clarify how many different templates were used. How were the templates chosen and how do they differ?
A3: Thanks for your insightful comments. For each environment, we designed several templates conveying different meanings, and then apply GPT to augment the languages. The detailed numbers are listed in the following table.
| Environment |Number of hindsight templates | Number of foresight templates | Number of augmented sentences for each template |
|---|---|---|---|
| HomeGrid | 20 | 9 | 70 |
| AlfWorld | 4 | 4 | 200  |
| Messenger | 4 | 4 | 200 |
| MetaWorld | 2 | 6 | 180  |
The templates were selected to provide agents with diverse types of privileged knowledge across various situations. For instance, in the Messenger environment, two specific foresight instructions illustrate this approach effectively.
|Foresight Instruction |Privileged knowledge |situation |
|---|---|---|
|“Move {action} to avoid the {enemy} at {loc}” |optimal action, enemy entity, enemy location | agent in danger |
|“Step {action} to approach the {target} at {loc}” |optimal action, target entity, target location | no enemies around | 
More examples can be seen in Appendix A. We appreciate your suggestion and will clarify these points in our revision. Thank you for your feedback.
Q4. How we compare the actions from the previous step and how exactly this comparison leads to choosing the template.
A4. Thank you for your perceptive question. In our implementation, we compare the agent’s actions with expert actions and analyze the agent’s task progress and situations. This allows us to determine whether the agent is on the right track and decide which type of privileged knowledge may help the agent. The template is then chosen based on this analysis, mimicking how humans assess situations and provide suggestions.
For example, in the Messenger environment, we compare actions, consider the locations of the target and nearest enemy, and generate hindsight reflections.
We apologize for any confusion and will elaborate more on this point in the revision.
Q5. We claim the generalizability over unseen tasks. However, the evaluation only contains one unseen task. More clarification is needed.
A5. Thank you for your insightful question. We will clarify that our current evaluation demonstrates generalization to one unseen task. In future work, we will study its generalization to a broader range of diverse unseen tasks.
If the above responses address your concerns, we hope you kindly consider raising the scores. Thank you!



Reviewer Po6y
Reviewer (Score 3.5)
We thank the reviewer for the positive feedback on the novelty of this work and its added value for understanding the role of language feedback in RL learning. We appreciate all the insightful questions, comments, and suggestions. 

Q1: Is there any guarantee that offline RL can converge to an optimal policy using the LTDT framework on sub-optimal trajectories? Does the LTDT agent achieve better or similar task performance compared to the sub-optimal/expert policy?
A1: Generally, offline RL trained on sub-optimal trajectories does not guarantee the achievement of an optimal policy. This limitation arises because offline RL assumes no further interaction with the environment to gather new trajectories, leading to issues such as low quality trajectories, limited exploration, and distribution shift. While offline RL can sometimes outperform sub-optimal policies, it is challenging for LTDT to perform at the same level when training data is limited, especially since our sub-optimal policies are actually optimal policies with some perturbed actions during interaction that still achieve nearly 100% success. 
Here are the performance results based on different training data sizes on the Messenger environment. The data size we use in the experiment is 20k. We test the performance of the baseline model trained without any languages.
|Data size | Performance|
|--|--|
|20k trajectories | 51.6%|
|50k trajectories |  71.2%|
|100k trajectories| 88%|
Our paper's primary goal is not to beat sub-optimal/optimal policies. Instead, we aim to study how natural language with different levels of informativeness and diversity during pre-training influences evaluation within a limited training budget. Therefore, we use a 10~20k data size across all our experiments. We will provide more explanation on this in the revised version. Thank you for your feedback!

Q2: How does the degree of divergence between expert and sub-optimal policy influence agent learning?
A2: Thank you for your insightful question. The sub-optimal policy is used for introducing some errors or perturbations in the training data, and letting the expert policy continue to recover. This helps agents learn to recover from potential failures using hindsight reflections and foresight instructions. In our experiments, we introduced 10-20% random noise in each trajectory as a sub-optimal policy. We found that this level of perturbation aids learning, but excessive disturbance (e.g., >50% per trajectory) significantly degrades performance as agents start learning suboptimal behaviors. 
Q3: All environments used in the paper are text-based environments.
A3: Sorry we didn’t clearly explain the environment in the paper. Actually, HomeGrid and MetaWorld are not entirely text-based; HomeGrid uses image observations for state inputs, and MetaWorld utilizes vectors that include information about the robot arm's position and status. More clear comparison is below and we will add this later.
|Env|image observation|instruction manual|state description|
|--|--|--|--|
|Messenger | no | yes | no| 
|HomeGrid| yes | no | no |
|MetaWorld| no | no | no |
|Alfworld| no | no | yes |

Q4: Are instruction manuals or state descriptions used in LTDT, in addition to the augmented language feedback? Why don't you use an Atari environment that has continuous action spaces?
A4: Yes, we use additional information, such as instruction manuals or state descriptions, if provided by the environment. The reason we did not choose continuous action spaces is two-fold: 1) Continuous actions are more challenging to describe using natural human language compared to discrete actions. 2) The Decision Transformer, which serves as the intrinsic architecture of LTDT, is not sufficiently compatible with predicting continuous actions. We plan to explore this area of research in future work.
Q5: Consider including other baselines like Dynalang and EMMA to enhance the significance of this work.
A5: Thank you for the suggestion! We will include these baselines in the revision. Compared to previous work, our focus is on how the informativeness and diversity of language can enhance model understanding of tasks and improve online performance, rather than proposing new architectures. However, we recognize the importance of including these methods as baselines and will conduct experiments with them in our future work. Thank you!

Q6: It seems unfair that agents are evaluated in the GPT-augmented foresight+hindsight condition, which is not the same setting as they are trained.
A6: Thank you for pointing this out! The reason we use online GPT for all evaluations in RQ1 and RQ2 is to mimic real-life human language environments and to determine whether agents trained with a higher level of language informativeness and diversity perform better in these environments. To address your concern, we also include the results of agents under different evaluation settings, as follows:

For RQ1, we run more experiments on HomeGrid environment
| Training language| Eval with the same type of language during training | Eval with Online GPT (original number in the paper)|
| -------- | ------- |------- |
| No Lang | 0.235  | 0.212 |
| Template Hindsight | 0.260 | 0.246 |
| Template Foresight | 0.305 | 0.262 |
| Template Hindsight + Foresight | 0.325 | 0.285 |
| GPT-augmented Hindsight + Foresight | 0.472 | 0.442 |

For RQ2 we run more experiments on Messenger environment
| Training language| Adapt and eval with the same type of language during training | Adapt with GPT-augmented foresight+hindsight languages and Eval with Online GPT (original number in the paper)|
| -------- | ------- |------- |
| No Lang | 0.323  | 0.270 |
| GPT-augmented Hindsight | 0.450 | 0.378 |
| GPT-augmented Foresight | 0.512 | 0.464 |
| GPT-augmented Hindsight + Foresight | 0.623 | 0.608 |



We find that aligning the informativeness and diversity levels between training, adaptation and evaluation improves the final performance for all types. However, even with aligned evaluation and adaptation language, no other settings have outperformed GPT-augmented Hindsight + Foresight evaluated with online GPT. This further demonstrates that high informativeness and diversity in language help agents understand tasks and achieve better performance. We will add complete results in the revision version, Thanks for the suggestion!



Q7: The motivation and conclusion of the ablation study are not made very clear. 
Q7.a: Fig. 6 needs more elaboration. 
A7.a: The motivation for this ablation study stems from the observation that language assistance does not always boost agent performance. We hypothesize this may relate to task difficulty, and we aim to identify when agents benefit most from language support.

Although the scatter plot appears to show a linear increase, many points on the right are at zero, obscured by the horizontal axis. This indicates that for very challenging tasks, efficiency gains may get zero, showing that language assistance is not effective enough to help agents achieve their goals in those cases. Therefore, we chose a 2-degree polynomial fit to better capture the trend of efficiency gain’s first increasing and then decreasing, and conclude that languages help agents most when the task difficulty is moderate.

Thank you for highlighting these issues. In our revision, we will clarify our motivations and revise the figures to avoid any confusion.
Q7.b: Counter-intuitive results for performance vs. language frequency.
A7.b: In our experiments, we use online GPT to decide whether to respond, aiming to mimic human behavior. However, this approach inevitably misses many crucial steps that are worth intervention, unlike real humans who can intervene only when necessary. As a result, we observe that increasing language frequency allows for capturing all crucial intervention steps, which explains why higher frequency leads to better performance.

	
Q7.c: The adversarial condition should perform worse than the empty condition if the agent follows the instruction strictly. 
A7.c: The adversarial condition performs better because the agent, pretrained with more informative and diverse language, can understand the task goal better and does not solely rely on instructions to take actions. The agent balances between noisy instructions and the clear task goal. A key underlying reason is that all instructions in our model are encoded by a sentence-BERT into embeddings. Compared to empty string instruction embeddings, the embeddings of adversarial instructions (drawn from GPT) still fall into a meaningful part of the semantic space close to the training embeddings. Despite the noise, LTDT can predict reasonable actions given these inputs. Conversely, inputting an empty instruction embedding, which is too far from the training embeddings, harms the agent's performance.
To further illustrate this, we include results with a zero embedding (zero vectors of the same size as sentence-BERT embeddings) and average embeddings (averages of all GPT-augmented template embeddings) on the HomeGrid environment below:

|Type|Reward|
|---|---|
|Empty instruction embedding| 0.32|
|Zero embedding|0.33|
|Average. embedding|0.33|
|Adversarial instruction embedding | 0.35|


If the above responses address your concerns, we hope you kindly consider raising the scores. Thank you!

Additional Rebuttal
Q1. The rationale for running the experiments about informativeness and diversity with 20k trajectories lacks explanation. Does the finding generalize to larger training budgets?
A1. Thank you for your perceptive comment. We chose a smaller data size for our experiments because collecting robotic datasets in real life is non-trivial, often limiting the scope of available data. Our goal is to investigate how applying language can augment limited data and determine which types of language can best boost the agent’s performance in a data-efficient manner.
We appreciate your suggestion and will test our findings with larger training budgets in future work.


Q2.  The evidence in Fig 6 is not strong enough to conclude the inverted-U shape relationship between task difficulty and gain. 

Q3.  Adversarial instructions are not adversarial enough to negatively impact the performance, but rather similar to the average / zero embeddings


Reviewer TLds (Score 2.5)
We appreciate the reviewer’s acknowledgment that “the work really raises and explores for the first time the question of the quality of language feedback in the learning of agents in the virtual environment. ” We thank the reviewer for the valuable comments and suggestions. 


While there is no new architecture, the novelty of this work lies in a systematic investigation of the role of different types of feedback in interactive RL learning. As the reviewer points out, this is the first time the question of language feedback in the learning of agents is explored. 


Q1: Lacking mention on IGLU and Dynalang.
A1: Thanks for pointing this out! We have cited Dynalang in the introduction but we didn’t include sufficient discussion about our work in relation to IGLU and Dynalang in the related work section. Here we elaborate on our main differences:
IGLU: There are two major differences:
We have separate taxonomies for the instructions. IGLU uses four types of help (Restrictive, Length-based, Corrective, Mistake-based), which are customized for MineCraft-like tasks. We use hindsight and foresight to measure informativeness and apply this to four different environments.
IGLU aims to teach RL agents how to seek proper types of help from online users and build a new Human-Centered AI Collaboration framework. Our work is mainly focused on studying the essential factors that will influence online performance when user feedback is available for agents pre-trained with different types of language feedback.
Dynalang: Dynalang focuses on building world models that can learn both language and actions. In contrast, we aim to answer how the informativeness and diversity of natural language used during RL training affect the decision-making ability of an agent. We chose the Decision Transformer for our experiments due to its adaptability to our problems. Dynalang uses a Recurrent State Space Model (RSSM) to build latent representations for language and the world, requiring Learning to Act by Latent Imagination, which is non-trivial to adapt to our problem.
We will add more discussions in the revised version. 

Q2: Needs to relate to the generation of scalar reward signals using LLM.
A2: In our paper, we focus on natural language as feedback for RL agents, a new paradigm in recent benchmarks such as LLF-bench. Our research centers on understanding the role of language in teaching agents during the training process, mimicking real interactions between humans and robots that are primarily based on natural language. Incorporating scalar rewards, code, action, or vector-based feedback are all interesting directions to pursue in the future. 

Q3: It seems important to experiment with giving different types of instructions only at the beginning of the task to the agent.
A3: We agree with the reviewer that there are different ways language can be explored in RL. Within the scope of this paper, we focus on “interactive” language use as it’s more aligned with teaching agents in action (i.e., through interactive feedback). Humans typically teach and interact with robots in an ongoing, dynamic manner. We  will leave non-interactive settings for future work.
Q4: More experiments with different quality of expert data.
A4: We appreciate the suggestion! While this is standard in offline RL, our focus is on understanding which aspects of natural language—such as diversity and informativeness—are crucial for teaching an RL agent. Given the scope of this paper, we chose expert data so we can have a better control across different configurations of language use. Quality of expert data will certainly add another rich dimension which we will explore in the future. 

Q5: Why adversarial feedback still performs well remains unclear.
A5: Sorry that we didn’t explain it clearly. A key underlying reason is that all instructions in our model are encoded by a sentence-BERT into embeddings. Compared to empty string instruction embeddings, the embeddings of adversarial instructions (drawn from GPT) still fall into a meaningful part of the semantic space close to the training embeddings. Despite the noise, LTDT can predict reasonable actions given these inputs. Conversely, inputting an empty instruction embedding, which is too far from the training embeddings, harms the agent's performance.
To further illustrate this, we include results with a zero embedding (zero vectors of the same size as sentence-BERT embeddings) and average embeddings (averages of all GPT-augmented template embeddings) on the HomeGrid environment below:

|Type|Reward|
|---|---|
|Empty instruction embedding| 0.32|
|Zero embedding|0.33|
|Average. embedding|0.33|
|Adversarial instruction embedding | 0.35|


If the above responses address your concerns, we hope you kindly consider raising the scores. Thank you!

It’s okay to send a confidential comment to AC as this reviewer seems to miss the main focus of this work. Many comments/suggestions,  although interesting,  are out of the scope of this work. 

Dear AC, although this reviewer recognized the novelty of this work (as they acknowledge that this is “the first time” the question of language feedback in RL learning agent is explored), they seem to miss the focus of this work (i.e., interactive language use).  Many comments/questions, although interesting,  are out of the scope of this work. Addressing them in this paper will dilute the current focus. We would like to respectively bring this to AC’s attention. 




